Anticipation of Method Execution in Mixed Consistency Systems -- Technical Report

Distributed applications often deal with data with different consistency requirements: while a post in a social network only requires weak consistency, the user balance in turn has strong correctness requirements, demanding mutations to be synchronised. To deal efficiently with sequences of operations on different replicas of the distributed application, it is useful to know which operations commute with others and thus, when can an operation not requiring synchronisation be anticipated wrt other requiring it, thus avoiding unnecessary waits. Herein we present a language-based static analysis to extract at compile-time from code information on which operations can commute with which other operations and thus get information that can be used by the run-time support to decide on call anticipations of operations in replicas without compromising consistency. We illustrate the formal analysis on several paradigmatic examples and briefly present a proof-of-concept implementation in Java.

==> evaluation.tex <==

\section{Use-Cases}\label{sec:evaluation}

We applied our approach and analysis to four common use-cases in the field.
%
The purpose is to illustrate how problems identified in recent papers may be solved in \model, and to provide insight on the output of our static analysis.

In this context, Table \ref{tab:results} presents statistics for each use-case, concerning:
\begin{inparadesc}
\item[the use of \model:]  
 number of weakly consistent fields, of field invariants, of methods; and
\item[the static analysis:]
 number of non-\textbf{LP} methods, of pairs of methods analyzed, of conflicts  detected, and the possible anticipations:
 
 Let $m_2$-$m_1(c)$ indicate that, given a sequence $m_1;m_2$, the method $m_2$ can anticipate $m_1$ when $c$ holds, thus giving rise to the sequence $m_2;m_1$.
\end{inparadesc}
%
In the remainder, we do to consider the cases whether
two calls of the same method on the same instance and with the same argument do commute.
%The code of the use-cases is available in~\S~\ref{sec:use-cases-code}.


\input{results}

\paragraph{Account}
Consider the example presented in Listing~\ref{lst:bank}. The results of the static analysis are:
\begin{description}
\item[non-LP methods:]
%\textbf{Static analysis}: \textit{Non-LP methods}: 
\texttt{transfer}, \texttt{withdraw}, \texttt{accrueInterest} (\texttt{acc}, for short).
%\textit{conflicts}
\item[conflicts:] when applied on the same account,

\texttt{init} (noted \texttt n) with all methods but \texttt{getBalance}; and each of \texttt{deposit}, \texttt{withdraw}, \texttt{transfer} and \texttt{\texttt{acc}} itself with \texttt{\texttt{acc}}.
%\textit{anticipations}
\item[anticipations:] \texttt{get\-Balance} can anticipate all method calls;
%and

- \texttt{deposit} can anticipate calls of LP methods;

- to anticipate \texttt{deposit} w.r.t. a non-LP method call, the two accounts must differ;

- to anticipate \texttt{acc}, the interest must be greater or equal~$-100$;

- when the call preceding \texttt{acc} is not a \texttt{getBalance}, the two accounts must differ; and

- to anticipate \texttt{init} when the preceding call is not a \texttt{getBalance}, the two accounts must differ.
\end{description}

\paragraph{Auction} An Ebay-like auction where bids and bidders
are weakly consistent, while  closing the auction is strong.
There are three replicated fields per auction item: the current bid, the bidder of the current bid, and a flag indicating if the auction is closed or open.
The example showcases how easy it is to write in \model the motivating example of coexisting weak bids and strong auction close operations, presented in~\cite{fgc-ATC2018}.
%
Both methods are transactions that operate over two replicated fields,
%being that, in this
so, in our implementation, all methods are locally permissible.

\medskip
The results of the static analysis are:
\begin{description}
\item[conflicts:] when applied upon the same auction,
\texttt{bid} with \texttt{bid} and 
\texttt{bidder} with \texttt{bidder}.
\item[anticipations:]
\texttt{bidder} and \texttt{bid} can anticipate each other; and

\texttt{bidder}, \texttt{bid} and \texttt{close} can be anticipated by all methods when the auctions are different.
\end{description}


\paragraph{Counter} An eventually consistent grows-only counter, on which increments are eventual, the read operation is strong, returning the
committed value of the counter.

\medskip
The results of the static analysis are:
\begin{description}
\item[non-LP methods:] none;
\item[conflicts:] \texttt{commit} with \texttt{inc}, when applied upon the same counter;
\item[anticipations:] \texttt{read} can anticipate other calls but \texttt{commit};

- \texttt{read} can be anticipated;

- \texttt{inc} can anticipate \texttt{inc}; and

- in all remaining cases, all methods can be anticipated when the counters are different.
\end{description}


\paragraph{Register}% A register
Let it be similar to the one available in Dynamo~\cite{dynamo-SOSP2007}, with strong and weak \textit{getter} operations over strong and weak registers, respectively, with increment and decrement operations, and with a commit operation to synchronize the register.

\medskip
The results of the static analysis are:
\begin{description}
\item[non-LP methods:] none;
\item[conflicts:] when applied on the same register,

- \texttt{commit} with \texttt{put}, \texttt{incr}) and \texttt{decr});

- \texttt{put} with \texttt{put}, \texttt{incr}, and \texttt{decr}.
\item[anticipations:] \texttt{get} can always anticipate, as well as be anticipated;

- \texttt{strongGet} can anticipate all calls but \texttt{commit}, as well as be anticipated;

- \texttt{incr} and \texttt{decr} can anticipate \texttt{incr} and \texttt{decr} and in all remaining cases;

- all methods are anticipable when the registers are different.
\end{description}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

==> language.tex <==
\section{The Language}
\label{sec:model}

%A key contribution of our work, which contrasts with the related work, is being language-based: we have a formal language with a rigorous semantics and the concepts are 
%implemented in Gallina and type-checked (hence, even setting the ground for mechanical verification).

%\paragraph{The Language}
\input{tab-selected-syntax}
The object-oriented language under consideration, 
dubbed \model-\oolong, is meant to model replicated systems where object fields are \textit{strongly consistent},
unless explicitly marked as weakly consistent.
%
We present in Table~\ref{tab:selected-syntax} the syntax of
\model-\oolong that increments~\cite{oolong-ACR2019};
the full syntax, and the (static and dynamic) semantics is available in
a companion technical report~\cite{sac23-tech-report}.
%\alarmAntonio{Produce bibitem}

\paragraph*{Syntax.}
%So, a
A field declaration, by default strongly consistent, can be optionally flagged with the \weakk keyword to indicate that the field has weak consistency. 
Field and method declarations are decorated with a (possibly empty) set of invariants~$c$, where in the latter case $c$ is often referred to as a precondition;
an invariant is an application of a binary predicate \Rel\ over integers.
%
Invariants are used solely for program analysis purposes 
(the call anticipation analysis of \S~~\ref{sec:conflicts} and
\S~\ref{sec:re-static-commutativity}),
and have no impact on the dynamic semantics. 

A value $v$ can be a \nullk~reference, an integer~$n$ or a location~$\iota$.
A novelty are 
%is the presence of
\emph{symbolic values}~$sv$ that include values, variables $x$ and applications of integers operators $\Op$ to symbolic values.
%
%As usual, occurrences of a variable $x$ are \emph{bound} in an expression $e_2$ in the context of a let-expression \kw{let} $x$ \c{=} $e_1$ \kw{in} $e_2$. Occurrences of other variables in $e_2$, or in general in an expression not inside a let are \emph{free}.

%Let~$x$ be in ${\sf fv}(e)$, the free variables of an expression~$e$,
%if there is at least an occurrence of~$x$ in~$e$ that is not bound by a let-expression,
%and $x\in{\sf bv}(e)$ when $x$ is bound by a let-expression in $e$.
%\alarmHerve{is this correct? shouldn't it be, "otherwise"?, i.e. all occurrences are bound}
%\alarmMarco{Not all occurrences are bound. 
%E.g. x in x.f is not bound, while x in let x = e in x.f is bound.
%The definition seems ok to me, please cross-check Hervé and Antonio}

\paragraph*{Semantics.}
The evaluation relation, noted $\Cfg\hookrightarrow \Cfg'$, recast the single-thread semantics of OOlong, 
modulo the presence of integer operations.
A configuration \Cfg\ is a pair $\langle \Sigma, e\rangle$ where $\Sigma$ is the {\it state}
and $e$ is an expression. 
A state contains an heap~$H$ mapping locations to objects, 
a stack $V$ mapping variables to values,  
and two extra-fields to {\it monitor} the method calls' preconditions 
and the access to strong fields, respectively.

The first extra-field monitors if an execution respected the meth\-od's preconditions:
e.g. if a method $m$ of class $C$ has the pre-condition $\thisk.f \geq 1$,
where $f$ is an integer field of $C$,  and $m$ is executed, 
then the first extra-field contains
the entry $n\geq 1$, where $n$ is the value of $\thisk.f$ at execution time;
%
by evaluating $n\geq 1$ \emph{after} the call's execution, 
we are able to infer if the call was legit.
%
The second extra-field contains entries of the form $(\iota, f, \kw r)$ and 
$(\iota, f, \kw w)$ indicating that
the strong field $f$ of the object in location $\iota$ has been accessed 
during the execution in \emph{read} and \emph{write} mode, respectively.

%\alarmAntonio{Unclear... Example?}

An object is a pair $(C,F)$, where $C$ is a class identifier and $F$ is a map from fields to values.

\paragraph*{Type System.}
The rules inductively define the typing relation $\Gamma\vdash e\colon t$.
%The typing rules for expressions are those of~\cite{oolong-ACR2019} 
The original rules for expressions~\cite{oolong-ACR2019} were
extended with rules for integers.
%
The rules for fields and methods enforce that 
an invariant $c$ of a field $f$ cannot refer to fields different from~$f$, and 
a precondition $c$ of a method cannot refer to weak fields, respectively.
%
The rules for configurations, noted as $\Gamma\vdash\Cfg\colon t$,
extend straightforwardly~\cite{oolong-ACR2019} by adding rules for the monitoring fields.




\begin{lstlisting}[caption=Bank account, label=lst:bank,float]
class Account implements Object {
  balance  : int weak [this.balance$\geq$0]
  min_cash : int [this.min_cash$\geq$50]
        
  def init (amount : int) : Unit [amount$\geq$this.min_cash]{ 
   this.balance = amount 
  }
         
  def withdraw(amount : int) : Unit [amount$>$0] { 
   this.balance -= amount  
  } 
        
  def transfer(recv : Transfer) : Unit {
   let a = recv.amount in let w = recv.account in
    this.withdraw(a); w.deposit(a) 
  }
        
  def deposit(amount : int) : Unit [amount$>$0] { 
   this.balance += amount
  } 
          
  def accrueInterest(interest : int) : Unit {
   let x = this.balance * interest / 100 in
    this.balance += x
  }
            
  def getBalance() : int  { this.balance }
  
}
\end{lstlisting}

\paragraph{Programming Example}
Listing~\ref{lst:bank} shows how to program  in \model-\oolong an account whose balance is replicated but does not require strong consistency.
Importantly, as intended, the code is identical to a non-replicated implementation.
The weak field \texttt{balance} cannot be mentioned in the methods' preconditions;
on contrast, the strong field \texttt{min\_cash} can be accessed in method \texttt{init}
to verify that the initial amount is greater or equal to the minimum allowed.
%
The state invariant is that of fields \texttt{balance} and \texttt{min\_cash}.
%\alarmHerve{motivate max\_cash}
Methods that do not change the state invariant are \textit{locally permissible} 
(cf.~\texttt{getBalance}), while a method~$m$ that may change the state invariant is locally permissible in a pre-state satisfying its invariants if and only if all calls of $m$ satisfying the preconditions spawned from the call lead to post-states that satisfy their invariants; for instance, a call $\texttt{transfer}(n)$ spawns the precondition $n>0$.
%
Therefore, methods \texttt{init} and \texttt{deposit} are locally 
permissible, since the amount to be initialized or deposited, respectively, 
must be positive, while \texttt{withdraw}, \texttt{transfer} and 
\texttt{accrueInterest} are not.% locally permissible.
    
    
%\paragraph{Method Call Execution}
\paragraph{\model method calls execute as indivisible units over the  target data}
In \S~\ref{sec:cs} we elaborate on the consistency level assigned to the execution of each method call.
For now, to make the presentation  of the following sections clearer, we simply state that method calls that either access strong fields or are not locally permissible require strong consistency semantics.
%
The remainder may execute under causal or even eventual consistency, depending on whether causality relations have been identified between  methods or not. 

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

==> re-static-commutativity.tex <==
\section{Static Analysis of Call Anticipation}
\label{sec:re-static-commutativity}

The notion of call anticipation introduced in the previous section relies on checks that are executed at \emph{runtime}; the use of constraint solving, in particular, comports that call anticipation cannot be effectively used, because of the latency of the decision process.

In this section, we develop a static analysis that mimics the construction 
of~\S~\ref{sec:conflicts} without relying on information that is only available at runtime. 
In the following, we present the concepts informally, 
and refer to the technical report~\cite{sac23-tech-report} 
for the formalization of the construction that makes the static analysis feasible.
%the  technical devices that make the static analysis feasible.

\subsection{Static semantics, informally}
The wedge of the theory introduced in~\S~\ref{sec:conflicts} 
is the execution of method calls. In \model-OOlong, executing a method call involves information that is only available at runtime:
i) the objects in the heap and the values of their fields;
ii) the instance calling the method;
iii) the actual parameter of the method.

\paragraph*{Executing methods}
The challenge that we attack in this paper is:
%whether it is possible to \emph{execute a method} rather than execute a method call
\begin{center}
    \emph{how to execute a method, rather than a method call}?
\end{center}
% that is, 
We are interested in devise a symbolic execution model where
methods can be executed irrespectively of %certain 
information %that is 
only available at runtime. 
The ultimate goal is to extract its side effects and reason 
about method commutativity and permissibility.
%
In order to do that, we provide the intuition of how we manage the missing information mentioned in items 
i), ii) and iii) outlined above.

To attack i), we rely on a \emph{symbolic heap} that contains the 
\emph{symbolic objects} that are needed for the execution of the method; crucially, these objects are symbolic since their (integer) fields at bootstrap have assigned uninstantiated variables rather than values, and can be generated automatically from class definitions.

To attack ii), we assume that a symbolic instance of the class of the method is available in the heap, and refer to %this instance
it as $\thisk$.

To attack iii), when the type of the parameter is a class, we proceed as in case ii) and assume that the parameter instance exists in the heap, and call it $\otherk$; otherwise, when the type of the parameter is an integer, we use the uninstantiated formal parameter of the method.

%In a nutshell, our symbolic execution model relies on the connection 
%structure of the objects referred by the instances 

\paragraph*{Boostrap heap}
The static analysis relies on a heap that is generated from a set of class definitions.
Given a class, we generate an instance by assigning 
fresh uninstantiated variables to integer fields,
and by generating instances assigned to object fields.

\paragraph*{Effects of expressions}
%As such, we have
Let us set up an infrastructure %that could be useful
to avoid relying on the actual values of methods and objects.
Still, we need to be able to reason on the modifications to objects that occur in the body of the method, that is, we need to execute (a representation of) the method.
%
To this aim, one key notion is that of symbolic value (productions $sv$ in Table~\ref{tab:selected-syntax}), %Symbolic values could be 
used to track the manipulations done to integer fields without relying on actual values.

To illustrate, consider method \texttt{deposit} of Listing~\ref{lst:bank}.
The behaviour of the body of the method can be expressed in terms of the modification of the symbolic heap 
$H$ below, where $x$ and $y$ are the symbolic variables assigned to 
the fields \texttt{balance} and \texttt{min\_cash} of $\thisk$ in $H$, respectively:
$$
H[\thisk\mapsto (\textit{Account}, (\texttt{balance}\mapsto x + \texttt{amount},
\texttt{min\_cash}\mapsto y))]
$$
Updating the instance of $\thisk$ comports that the field \texttt{balance}
has assigned the symbolic value
$x + \texttt{amount}$, where \texttt{amount} is the formal parameter of 
\texttt{deposit}.

To obtain this modification, we need to be able to evaluate the \textit{effect}
of the body of the method, that is the effect of expressions.
%
To this aim, we cannot rely on the evaluation of expressions in \model-\oolong,
which not only requires actual values, but also evaluation contexts.
%, which suit poorly our objectives.
%
Instead, we represent the effect of an expression as a list of constructors %that provide
capturing the expression functionality;
note that the \emph{flat} structure of effects allows efficient calculation of the modifications done to the symbolic memory by relying on a single slot for \emph{return values} that acts as a buffer.

\paragraph*{Calculation of effects.} Rules have the form $\Gamma\vdash e\ret E$, where $\Gamma$ is the type environment
and $E$ is the produced effect list, inductively defining  the function extracting the side effects of an expression.
Rather than discussing the syntax of effects and their inference rules
(available in~\cite{sac23-tech-report}),
we draw the intuition of their usage with an example.
%\alarmAntonio{Where are the rules?}
%
Consider method \texttt{deposit} of Listing~\ref{lst:bank}.
The effect of a method is the effect of its body, which is calculated giving in 
input the environment that is used to type-check its body, and the body expression, 
and receiving in output an effect list.
%For instance, in the case of the body of \texttt{deposit}, the calculated effect. given 
That is, when $\Gamma=\thisk\colon\textit{Account},\texttt{amount}\colon\intk$,
the effect of \texttt{deposit} is:
$$
\Gamma\vdash \thisk.\texttt{balance}\, \c{+=} \, \texttt{amount}\ret E_1 \circ [\ottkw{Evar}(\ottkw{Vfield}(\thisk,\texttt{balance}))]
$$
where  the last entry of $E_1$ is $\ottkw{Eop}(+,\texttt{amount})$,
the remainder of $E_1$ contains constructors that will load the symbolic value~$x$ 
of field \texttt{balance} into the buffer,
and $\circ$ indicates list concatenation.
%
By executing $\ottkw{Eop}(+,\texttt{amount})$, the buffer is set to
the symbolic value $x+\texttt{amount}$; %the execution of
executing
$[\ottkw{Evar}(\ottkw{Vfield}(\thisk,\texttt{balance}))]$ assigns the symbolic value of the buffer to the field \texttt{balance} of $\thisk$.

\paragraph*{Methods Commutativity}
To establish the conditions under which two methods $m_1$ and $m_2$ commute, 
we symbolically execute method $m_1$ followed by method $m_2$, noted $m_1;m_2$, 
and vice versa,  and inspect the symbolic heaps obtained by the executions 
$m_1;m_2$ and $m_2;m_1$: by equating the two heaps \emph{field-by-field} we obtain
an integer constraint system that set the conditions under which the two methods commute.
%
The integer constraint system contains
the constraints $eqs$ equating the heaps $H_1$ and $H_2$, and the constraints
$\tilde c$ generated by the fields' invariants and methods' preconditions. 
We note that a method execution $m_1;m_2$ can be seen as a \emph{sequence} since 
$m_2$ is executed w.r.t. the heap modified by $m_1$. 

%
Crucially, the bootstrap heap must contain the objects 
manipulated by the two methods; that is, we need to generate the heap by passing the
classes of the two methods, and the classes of their parameters.
When a class appears more than once, whether we need to create more instances depends
on \emph{aliasing}: that is, the heap generation must takes into account whether 
two or more instances of a same class are indeed an alias of the same object.

To manage aliasing, we need to parametrize our analysis w.r.t. the identity of the 
(addresses of the) instances occurring in the two methods, noted $\doteq$.
In general, there are least two objects, the instance of $m_1$, noted $\thisk_1$, 
and the instance of $m_2$, noted $\thisk_2$.
Moreover, each method $m_i$ can have an object parameter, noted as $\otherk_i$, $i=1,2$.
Depending on the class of the objects and on their identity, we have at most 
fifteen possible cases
in terms of equality and disequality, e.g. 
1) $\thisk_1\doteq\thisk_2$ and $\thisk_2 \doteq \otherk_1$ and
$\otherk_1 \doteq\otherk_2$, or
6) $\thisk_1 \doteq\thisk_2$ and $\otherk_1 \doteq\otherk_2$, and so on,
where the absence of an equality among two instances means that they do differ.
Thus, in case 1) the bootstrap heap will contain \emph{at least} one instance,
while in case 6) the heap will contain at least two instances.


%Commutativity is parametric w.r.t. conditions that allow the heaps generated by $m_1;m_2$ and $m_2;m_1$
%to be equated.

To illustrate, consider methods \texttt{deposit} and \texttt{accrueInterest} of 
Listing~\ref{lst:bank}, and let $\texttt a $ and $\texttt i$ abbreviate the formal 
parameters of \texttt{deposit} and \texttt{accrueInterest}, respectively.
We want to decide the conditions under which the two methods commute, expressed
in terms of the aliasing of the methods' instances and 
the integer constraints of the fields and of the methods' parameters.

The first thing to do is to set-up the aliasing conditions.  
In this example, the formal parameters are not objects, and in turn we only have two possible cases:
$\thisk_1\doteq\thisk_2$, and  $\thisk_1\not\doteq\thisk_2$.
In general, the presence of aliasing comports a more discriminating commutative analysis, 
so  let's consider the case whether the two methods are 
called on the same instance, named $\thisk$.
%
Assume that the bootstrap heap $H$ assigns to the field 
\texttt{balance} of $\thisk$ the variable~$x$.
The execution of the sequence \texttt{deposit};\texttt{accrueInterest} in $H$ gives rise 
to an heap $H_1$ s. t. the field 
\texttt{balance} of $\thisk$ has assigned the symbolic value 
$x +\texttt{a} + (x +\texttt{a})/100*\texttt{i}$,
while the execution of sequence \texttt{accrueInterest};\texttt{deposit} in $H$ gives rise
to an heap $H_2$ s.t. the field 
\texttt{balance} of $\thisk$ has value 
$x + x /100*\texttt{i} + \texttt{a}$.
%The integer constraint system generated by the commutative analysis contains
%the constraints $eqs$ equating the heaps $H_1$ and $H_2$, and the constraints
%$\tilde c$ generated by the field invariants and method preconditions. 
In particular, we have that the constraints $eqs$ equating the heaps $H_1$ and $H_2$ 
contain $\phi_1 \triangleq x +\texttt{a} + (x +\texttt{a})/100*\texttt{i} =
x + x /100*\texttt{i} + \texttt{a}$, while the field invariants and 
method preconditions $\tilde c$ contain
$\phi_2\triangleq x\geq 0$ and $\phi_3\triangleq\texttt a >0$. 
Since the constraint $\phi_1\land\phi_2\land\phi_3$ is not satisfiable, we conclude that methods \texttt{deposit} and \texttt{accrueInterest} do not commute when called on the same instance.
%On contrast, by considering a bootstrap heap with two different instances 
%$\thisk_1$ and $\thisk_2$ of methods \texttt{deposit} and \texttt{accrueInterest}, respectively,
%and by performing the commutative analysis, we obtain that the 
%methods commute under the constraint system 
%$x_1\geq 0$, $x_2\geq 0 and $\texttt a >0$. 

\paragraph*{Local Permissibility, statically}
We recast the predicates of~\S~\ref{sec:conflicts} in terms of the symbolic 
execution system.
We start by casting the \emph{runtime} notion of permissibility of method calls into a 
notion that can be decided \emph{statically}.

Remember that permissibility established at runtime requires:
i) a heap, and a stack;
ii) the actual instance of the call of a method;
iii) the actual parameter of the call of a method;
and that permissibility holds when, if the heap preserves the invariants of its fields,
and the call is guarded, 
then the post-heap obtained by executing the call still preserves the invariants of its fields.

In contrast, we statically analyze the behavior of the method,
rather than its call, by: (1) \emph{generating} a symbolic heap containing a symbolic instance of the class of the method, and the \emph{effect} of the body of the method;
and (2) by requiring the permissibility conditions of~\S~\ref{sec:conflicts},
now expressed in terms of the symbolic heaps and of the method's invariants.
%
In detail, we generate the constraints for the \emph{permissibility of a method} with the following  steps:
%\alarmAntonio{Why these steps?}
\begin{enumerate}
\item generate the boostrap heap $H_1$ w.r.t. the equality case under analysis 
($\thisk\doteq\otherk$ or  $\thisk\not\doteq\otherk$)
\item generate the effect of the body of the method and execute it w.r.t. $H_1$,
giving rise to the heap $H_2$
\item produce the constraint $\kw{inv}(H_1) \land {\tilde c}$ 
implies $\kw{inv}(H_2)$,
where $\kw{inv}(H_i)$ contains the field invariants of the heap $H_i$, $i=1,2$,
and $\tilde c$ are the closure of the methods' preconditions
\end{enumerate}
%
Dually, the steps to generate the conditions for 
\emph{non-permissibility of a method} are 1), 2), and the production of the constraint:
$$
\kw{inv}(H_1) \land {\tilde c} \text{ implies }\neg\kw{inv}(H_2)\, .
$$
%
To illustrate, consider methods \texttt{deposit} and \texttt{withdraw} of Listing~\ref{lst:bank}.
For what concerns \texttt{deposit}, as discussed earlier, 
steps 1) and 2) produce an environment $H_2$ s.t.
the field \texttt{balance} of $\thisk$ has the symbolic value $x + \texttt{amount}$, 
where $x$ is the value of  \texttt{balance} in $H_1$.
The permissibility analysis produces the formula
\begin{center}
$\phi_{\texttt d}\triangleq x \geq 0\land \texttt{amount} > 0\Rightarrow x + \texttt{amount}\geq 0$,
\end{center}
\noindent
which is satisfied for any value of $x$ and \texttt{amount}.
 Thus, \texttt{deposit} is permissible \emph{in all executions}.
Differently, by executing the steps for \texttt{withdraw}, 
we obtain the permissibility formula 
\begin{center}
$\phi_{\texttt w}\triangleq 
x \geq 0\land \texttt{amount} > 0\Rightarrow x - \texttt{amount}\geq 0$, 
\end{center}
\noindent
which is satisfied when $x\geq \texttt{amount}$.
Thus, \texttt{withdraw} is permissible when $x\geq \texttt{amount}$.

\emph{Local permissibility of a method} requires that permissibility holds for all possible values of 
the variables occurring in the formula.
The local permissibility formulas of \texttt{deposit} and \texttt{withdraw}
are, respectively: $\forall x,\texttt{amount}\,.\,\phi_{\texttt d}$
and
$\forall x,\texttt{amount}\,.\,\phi_{\texttt w}$;
since the former  is satisfiable 
%(\emph{SAT}, from now on) 
and
the latter is not satisfiable,
 %(\emph{UNSAT}, from now on),
we obtain that \texttt{deposit} is locally permissible while 
\texttt{withdraw} is not.


\paragraph*{Method Anticipation}
The objective of the static analysis of this section is to generate 
an integer constraint system that sets the conditions under which 
we can anticipate a call of a method $m_2$ w.r.t. the call of a method $m_1$
given an aliasing case $\hcase$ equating the addresses of the instances 
$\thisk_1,\otherk_1$ of $m_1$ and $\thisk_2,\otherk_2$ of $m_2$.
%
We already encountered a part of these constraints:
\begin{enumerate}
\item the constraint system $eqs\land \tilde c$ 
for the commutativity of $m_1$ and $m_2$ w.r.t. the bootstrap heap $H_1$ generated from 
\hcase
\item the local permissibility formula $\phi^{LP}_2$ of $m_2$ w.r.t. $H_1$    
\end{enumerate}
The remainder of the constraints contains a \emph{disjunctive} formula 
$\phi^{Or}_1$ 
setting the conditions for the permissibility of $m_1$ w.r.t. the heap $H_2$ reached by executing 
$m_2$ in $H_1$,
and an implication $\phi_{\texttt{ni}}$ setting the conditions for the 
\emph{non-interference} among the strong fields read by $m_2$ and written by $m_1$:
\begin{enumerate}
    \setcounter{enumi}{2}
     \item $\phi^{Or}_1\triangleq \psi^{LP}_1\vee \psi^{Pres}_1$, where 
     $\psi^{LP}_1$ is the local permissibility formula of $m_1$ w.r.t. $H_2$, 
     and
     $\psi^{Pres}_1$ is a conjunction of implications quantified over 
     all variables occurring in the weak fields of $H_1$:
     the permissibility of $m_1$ in the bootstrap heap $H_1$ implies
     the permissibility of $m_1$ in the post-heap $H_2$, and
     the non-permissibility of $m_1$ in the bootstrap heap $H_1$ implies
     the non-permissibility of $m_1$ in the post-heap $H_2$
    % $\psi^P_{\texttt m_1,H_1}$ implies 
    % $\psi^P_{\texttt m_1,H_2}$ and
    % $\psi^{NP}_{\texttt m_1,H_1}$ implies 
    % $\psi^{NP}_{\texttt m_1,H_2}$,
    % where $\psi^P_{\texttt m_1,H_i}$ and
    % $\psi^{NP}_{\texttt m_1,H_i}$ are the permissibility and non-permissibility
    % formulas of $m_1$ w.r.t. $H_i$, respectively, $i=1,2$
    \item $\phi_{\texttt{ni}}$ holds when in the execution $m_1;m_2$ w.r.t. the bootstrap heap $H_1$,
    if $(\iota,f,\kw r)$ is in the strong fields
    accessed by $m_2$  then 
    $(\iota,f,\kw w)$ is not in the strong fields
    accessed by $m_1$
\end{enumerate}

Item 3) sets the conditions to postpone $m_1$:
if $m_1$ is locally permissible in the post-heap $H_2$, %we have done, since 
no coordination is needed.
Otherwise, for all possible weak variables,
$m_1$ must preserve permissibility and non-permissibility w.r.t.
the bootstrap heap and the post-heap.
To better understand the discussion initiated in~\S~\ref{sec:conflicts} 
about why quantified preservation is mandatory, consider the case whether, in Listing~\ref{lst:bank}, we have a \texttt{withdraw} followed by a \texttt{deposit}, and we wish to anticipate \texttt{deposit}.
A \texttt{withdraw} could be not-permissible in one replica, 
and permissible in another replica, because the required amount 
is greater of the  weak value of \texttt{balance} in the first replica and 
less or equal in the second replica.
When trying to  anticipate \texttt{deposit}, quantified preservation would require that
the \texttt{withdraw} executed after the \texttt{deposit} in the first replica 
should still be not-permissible for all possible bootstrap values of 
\texttt{balance}, otherwise the two replicas would diverge after performing the call anticipation.
Since this clearly does not hold, by means of item 3) we rule out the possibility to anticipate \texttt{deposit} w.r.t. \texttt{withdraw} when the two methods are called on the same instance.


==> results.tex <==
\begin{table}[t]
  \caption{Statistics on the use-cases. }
\label{tab:results}
\resizebox{\linewidth}{!}{
\begin{tabular}{l||r|r|r|r
    ||r|r|r}
\multirow{2}{*}{\textbf{Use-case}} & 
\multirow{2}{*}{\# \weakk} & 
\multirow{2}{*}{\#   \textbf{invs}}   & 
\multirow{2}{*}{\#  \textbf{mtds}} & 
\multirow{2}{*}{\#  \textbf{non-LP}}   & 
\multirow{2}{*}{\# \textbf{pairs}} &
\multirow{2}{*}{\# \textbf{conflicts}} &
\multirow{2}{*}{\# \textbf{anticipations} $\dagger$\,($\thisk_1\not\doteq\thisk_2$)} 
\\
&   &  &  &     & &
\\        
\hline
  Account    & 1 & 2 & 6 & 3 & 15 & 9 
                                   &\texttt a-\texttt g~$(i\geq
                                     -100)$,
                                      \texttt a-\texttt d~$\ddagger$,
                                     \texttt a-\texttt t~$\ddagger$,
\texttt a-\texttt w~$\ddagger$,
                                     \texttt a-\texttt a~$\ddagger$, 
                                     \texttt a-\texttt n~$\ddagger$,\\
    &   &  &  &     & &&                                      
                                     \texttt g-\texttt *,
                                     \texttt n-\texttt g,
                                     \texttt d-\texttt g,
                                     
                                     \texttt d-\texttt d,
                                     \texttt d-\texttt a$\dagger$,
 \texttt d-\texttt w$\dagger$,
 \texttt d-\texttt t$\dagger$,
 \texttt d-\texttt n$\dagger$
  \\
  &   &  &  &     & &&
                                        \ $\ddagger\, (\thisk_1\not\doteq\thisk_2\land i_2\geq -100)$ 
\\
\hline
  Auction & 2 & 3 & 4 & 0  & 6 & 2 
                                           &\texttt{d}-\texttt{r},
                                             \texttt{r}-\texttt{d},
                                             \texttt{r}-\texttt{r}$\dagger$,
                                             \texttt{d}-\texttt{d}$\dagger$,
                                             \texttt c-\texttt{*}$\dagger$,
                                             \texttt *-\texttt{c}$\dagger$
                             
\\
\hline
  Counter & 1 & 0 & 3 & 0 & 3 & 1  
                                           &
                                           %\texttt c-\texttt c,
                                           \texttt *-\texttt  r,
                                             \texttt r-\texttt i,
                                             \texttt r-\texttt r,
                                             \texttt i-\texttt i,
                                             \texttt c-\texttt c$\dagger$,
                                             \texttt r-\texttt c$\dagger$,
                                             \texttt c-\texttt i$\dagger$,
                                             \texttt i-\texttt c$\dagger$
\\
\hline
  Register & 1 & 0 & 6 & 0 & 15 & 6 
  &\texttt *-\texttt g, \texttt *-\texttt s,
   \texttt g-\texttt *, \texttt s-\texttt i, 
   \texttt s-\texttt g, 
   \texttt s-\texttt d, 
   \texttt s-\texttt c$\dagger$,
   \texttt i-\texttt i,
    \texttt i-\texttt d, \\
& & & & & & &                                \texttt i-\texttt c$\dagger$,
    \texttt d-\texttt d, 
    \texttt d-\texttt i,
    \texttt d-\texttt c$\dagger$,
    \texttt c-\texttt *$\dagger$,
    \texttt p-\texttt *$\dagger$,
    \texttt *-\texttt p$\dagger$
    \\
  \hline
\end{tabular}
}
\end{table}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

==> tab-selected-syntax.tex <==
%\vspace{-2.5em}
\begin{table}[t]
\centering
  \caption{Selected syntax of \model-\oolong programs.
    %\textit{Ids, Cds, Fds, Mds and Msigs} are sequences of zero or
    %more of their singular counterparts.
    Terms in grey background are only available at
  runtime.}
\label{tab:selected-syntax}
%\resizebox{.9\textwidth}{!}{
\begin{tabular}{lcl}
  %\Rel & $::=$ & $<$ $~|~$ $\leq$ $~|~$ $\geq$ $~|~$ $>$ $~|~$ =
  %\hfill \textit{(Binary relations)}
  %\\
  $d$ & $::=$ & $x$ $~|~$ $x.f$  $~|~$ $v$ 
  \hfill \textit{(Invariant values)}
  \\
  $c$ & $::=$ & 
  %$\truek$ $~|~$ \weakk $x.f$ $~|~$ 
  $d_1 \ \Rel\  d_2$ 
  %$~|~$ $c_1 \land c_2$ $~|~$  
  %\\
  %&& $c_1 \vee c_2$$~|~$ $\neg c$ 
  \qquad\qquad\hfill \textit{(Invariants)}
  \\
  \Md & $::=$ & 
$m(x : t_1) : t_2$ $[\tilde c]$ \SB$e$\FB
  \hfill \textit{(Methods)}\\
  \Fd & $::=$ & $f : t \sim\hspace{-.2em}\weakk~[\tilde c]$ \hfill \textit{(Fields)} \\
  % \Md & $::=$ & \kw{def} \Msig \SB$e$\FB
  %               %$~|~$ \kw{def}\ \kw{rec} \Msig \SB$e$\FB
  %               \hfill \textit{(Methods)} \\
  $e$ & $::=$ & $sv$
        $~|~$ $x.f$
        $~|~$ $x.f$ \c{=} $e$
        $~|~$ $x.m(e)$ 
         $~|~$    \\
         &&\kw{let} $x$ \c{=} $e_1$ \kw{in} $e_2$
        $~|~$ \kw{new} $C$
        $~|~$ $(t)~e$\qquad\qquad
        \hfill \textit{(Expressions)} 
      \\
  $v$ & $::=$ & 
  \kw{null}
  $~|~$ $n\in\intk$
  %$~|~$ $-1$ $~|~$  $0$ $~|~$  $1$ $~|~$ \dots 
  $~|~$ \colorbox{lightgray}{$\iota$} \hfill \textit{(Values)} \\
  $sv$ & $::=$ & $v$
  $~|~$ 
  $x$
  $~|~$ $sv_1 ~ \ottnt{Op} ~ sv_2$
  \hfill \textit{(Symbolic Values)} \\
  %$\ottnt{op}$ & $::=$ & $+$ $~|~$ $-$ $~|~$ $*$ $~|~$ $/$  \hfill \textit{(Integer Operators)}\\
   $t$ & $::=$ & $I$ $~|~$ $C$ $~|~$ $\mathbf{Unit}$ $~|~$ $\intk$\hfill
                 \textit{(Types)}
                 \\
                 $\Gamma$ & $::=$ & $\epsilon$
  $~|~$ $\Gamma, x : t$
  $~|~$ \colorbox{lightgray}{$\Gamma, \iota : C$} \hfill
                     \textit{(Typing Environment)}
  %                    \\
  %   \colorbox{lightgray}{$\Cfg$} & $::=$ & $\langle H, V, \sff, \tilde c, ST\rangle$\qquad\qquad\qquad \hfill \textit{ { (Configuration)}}
  %   \\
  %   \colorbox{lightgray}{$H$} & $::=$ & $\epsilon$ $~|~$ $H, \iota \mapsto \obj$\hfill \textit{ { (Heap)}}
  %   \\
  %   \colorbox{lightgray}{$V$} & $::=$ &$\epsilon$ $~|~$ $V, x \mapsto v$\hfill  {\textit{(Stack)}}
  %   \\
  % \colorbox{lightgray}{$\sff$}& $::=$ & $\epsilon$ $~|~$ $\sff,(\iota, f)$\hfill
  %                  {\textit{(Strong fields)}}
  %   \\
  %   \colorbox{lightgray}{$ST$} & $::=$ &$e$ $~|~$ $\kw{EXN}$\hfill  {\textit{(Single Threads)}}
  %   \\
  %   \colorbox{lightgray}{$\obj$} & $::=$ &$(C, F)$\hfill  {\textit{(Objects)}}
  %   \\
  %   \colorbox{lightgray}{$F$} &$::=$ &$\epsilon$ $~|~$ $F, f \mapsto v$\hfill  {\textit{(Field map)}}
\end{tabular}
%}
\end{table}

 %%% Local Variables:
  %%% mode: latex
  %%% TeX-master: "main"
  %%% End:


